The sign rule and beyond: Boundary effects, flexibility, and noise correlations in neural population codes

Over repeat presentations of the same stimulus, sensory neurons show variable responses. This "noise" is typically correlated between pairs of cells, and a question with rich history in neuroscience is how these noise correlations impact the population's ability to encode the stimulus. Here, we consider a very general setting for population coding, investigating how information varies as a function of noise correlations, with all other aspects of the problem - neural tuning curves, etc. - held fixed. This work yields unifying insights into the role of noise correlations. These are summarized in the form of theorems, and illustrated with numerical examples involving neurons with diverse tuning curves. Our main contributions are as follows. (1) We generalize previous results to prove a sign rule (SR) - if noise correlations between pairs of neurons have opposite signs vs. their signal correlations, then coding performance will improve compared to the independent case. This holds for three different metrics of coding performance, and for arbitrary tuning curves and levels of heterogeneity. This generality is true for our other results as well. (2) As also pointed out in the literature, the SR does not provide a necessary condition for good coding. We show that a diverse set of correlation structures can improve coding. Many of these violate the SR, as do experimentally observed correlations. There is structure to this diversity: we prove that the optimal correlation structures must lie on boundaries of the possible set of noise correlations. (3) We provide a novel set of necessary and sufficient conditions, under which the coding performance (in the presence of noise) will be as good as it would be if there were no noise present at all.

==> usr_command.tex <==
% bold Latin
\newcommand{\bfone}{\mathbf{1}}
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}
% tilde Latin
\newcommand{\At}{\tilde{A}}
\newcommand{\Bt}{\tilde{B}}
\newcommand{\Ct}{\tilde{C}}
\newcommand{\Dt}{\tilde{D}}
\newcommand{\Et}{\tilde{E}}
\newcommand{\Ft}{\tilde{F}}
\newcommand{\Gt}{\tilde{G}}
\newcommand{\Ht}{\tilde{H}}
\newcommand{\It}{\tilde{I}}
\newcommand{\Jt}{\tilde{J}}
\newcommand{\Kt}{\tilde{K}}
\newcommand{\Lt}{\tilde{L}}
\newcommand{\Mt}{\tilde{M}}
\newcommand{\Nt}{\tilde{N}}
\newcommand{\Ot}{\tilde{O}}
\newcommand{\Pt}{\tilde{P}}
\newcommand{\Qt}{\tilde{Q}}
\newcommand{\Rt}{\tilde{R}}
\newcommand{\St}{\tilde{S}}
\newcommand{\Tt}{\tilde{T}}
\newcommand{\Ut}{\tilde{U}}
\newcommand{\Vt}{\tilde{V}}
\newcommand{\Wt}{\tilde{W}}
\newcommand{\Xt}{\tilde{X}}
\newcommand{\Yt}{\tilde{Y}}
\newcommand{\Zt}{\tilde{Z}}
\newcommand{\at}{\tilde{a}}
\newcommand{\bt}{\tilde{b}}
\newcommand{\ct}{\tilde{c}}
\newcommand{\dt}{\tilde{d}}
\newcommand{\et}{\tilde{e}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\gt}{\tilde{g}}
\newcommand{\htt}{\tilde{h}} % avoid conflict with \ht
\newcommand{\itt}{\tilde{i}} % avoid conflict with \it
\newcommand{\jt}{\tilde{j}}
\newcommand{\kt}{\tilde{k}}
\newcommand{\lt}{\tilde{l}}
\newcommand{\mt}{\tilde{m}}
\newcommand{\nt}{\tilde{n}}
\newcommand{\ot}{\tilde{o}}
\newcommand{\pt}{\tilde{p}}
\newcommand{\qt}{\tilde{q}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\st}{\tilde{s}}
\newcommand{\ttt}{\tilde{t}}  % avoid conflict with \tt
\newcommand{\ut}{\tilde{u}}
\newcommand{\vt}{\tilde{v}}
\newcommand{\wt}{\tilde{w}}
\newcommand{\xt}{\tilde{x}}
\newcommand{\yt}{\tilde{y}}
\newcommand{\zt}{\tilde{z}}
% bold tilde Latin
\newcommand{\bfAt}{\mathbf{\tilde{A}}}
\newcommand{\bfBt}{\mathbf{\tilde{B}}}
\newcommand{\bfCt}{\mathbf{\tilde{C}}}
\newcommand{\bfDt}{\mathbf{\tilde{D}}}
\newcommand{\bfEt}{\mathbf{\tilde{E}}}
\newcommand{\bfFt}{\mathbf{\tilde{F}}}
\newcommand{\bfGt}{\mathbf{\tilde{G}}}
\newcommand{\bfHt}{\mathbf{\tilde{H}}}
\newcommand{\bfIt}{\mathbf{\tilde{I}}}
\newcommand{\bfJt}{\mathbf{\tilde{J}}}
\newcommand{\bfKt}{\mathbf{\tilde{K}}}
\newcommand{\bfLt}{\mathbf{\tilde{L}}}
\newcommand{\bfMt}{\mathbf{\tilde{M}}}
\newcommand{\bfNt}{\mathbf{\tilde{N}}}
\newcommand{\bfOt}{\mathbf{\tilde{O}}}
\newcommand{\bfPt}{\mathbf{\tilde{P}}}
\newcommand{\bfQt}{\mathbf{\tilde{Q}}}
\newcommand{\bfRt}{\mathbf{\tilde{R}}}
\newcommand{\bfSt}{\mathbf{\tilde{S}}}
\newcommand{\bfTt}{\mathbf{\tilde{T}}}
\newcommand{\bfUt}{\mathbf{\tilde{U}}}
\newcommand{\bfVt}{\mathbf{\tilde{V}}}
\newcommand{\bfWt}{\mathbf{\tilde{W}}}
\newcommand{\bfXt}{\mathbf{\tilde{X}}}
\newcommand{\bfYt}{\mathbf{\tilde{Y}}}
\newcommand{\bfZt}{\mathbf{\tilde{Z}}}
\newcommand{\bfat}{\mathbf{\tilde{a}}}
\newcommand{\bfbt}{\mathbf{\tilde{b}}}
\newcommand{\bfct}{\mathbf{\tilde{c}}}
\newcommand{\bfdt}{\mathbf{\tilde{d}}}
\newcommand{\bfet}{\mathbf{\tilde{e}}}
\newcommand{\bfft}{\mathbf{\tilde{f}}}
\newcommand{\bfgt}{\mathbf{\tilde{g}}}
\newcommand{\bfht}{\mathbf{\tilde{h}}}
\newcommand{\bfit}{\mathbf{\tilde{i}}}
\newcommand{\bfjt}{\mathbf{\tilde{j}}}
\newcommand{\bfkt}{\mathbf{\tilde{k}}}
\newcommand{\bflt}{\mathbf{\tilde{l}}}
\newcommand{\bfmt}{\mathbf{\tilde{m}}}
\newcommand{\bfnt}{\mathbf{\tilde{n}}}
\newcommand{\bfot}{\mathbf{\tilde{o}}}
\newcommand{\bfpt}{\mathbf{\tilde{p}}}
\newcommand{\bfqt}{\mathbf{\tilde{q}}}
\newcommand{\bfrt}{\mathbf{\tilde{r}}}
\newcommand{\bfst}{\mathbf{\tilde{s}}}
\newcommand{\bftt}{\mathbf{\tilde{t}}}
\newcommand{\bfut}{\mathbf{\tilde{u}}}
\newcommand{\bfvt}{\mathbf{\tilde{v}}}
\newcommand{\bfwt}{\mathbf{\tilde{w}}}
\newcommand{\bfxt}{\mathbf{\tilde{x}}}
\newcommand{\bfyt}{\mathbf{\tilde{y}}}
\newcommand{\bfzt}{\mathbf{\tilde{z}}}
% Greek
\newcommand{\ka}{\kappa}
\newcommand{\ga}{\gamma}
\newcommand{\om}{\omega}
\newcommand{\tht}{\theta}
\newcommand{\eps}{\epsilon}
\newcommand{\mut}{\tilde{\mu}}
\newcommand{\bfeta}{{\boldsymbol\eta}}
\newcommand{\bfrho}{{\boldsymbol\rho}}
\newcommand{\bfmu}{{\boldsymbol\mu}}
\newcommand{\bfLambda}{{\boldsymbol\Lambda}}
\newcommand{\bfTheta}{{\boldsymbol\Theta}}
\newcommand{\bfSigma}{{\boldsymbol\Sigma}}
\newcommand{\bfxi}{{\boldsymbol\xi}}
\newcommand{\bfxit}{{\boldsymbol{\tilde{\xi}}}}
% control command
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\barr}{\begin{array}}
\newcommand{\earr}{\end{array}}
\newcommand{\beqr}{\begin{eqnarray}}
\newcommand{\eeqr}{\end{eqnarray}}
\newcommand{\beqrn}{\begin{eqnarray*}}
\newcommand{\eeqrn}{\end{eqnarray*}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}
\newcommand{\bei}{\begin{itemize}}
\newcommand{\beii}{\begin{itemize} \item}
\newcommand{\eei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bes}{\begin{small}}
\newcommand{\ees}{\end{small}}
\newcommand{\bec}{\begin{center}}
\newcommand{\eec}{\end{center}}
\newcommand{\betab}{\begin{tabular}}
\newcommand{\eetab}{\end{tabular}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}{Claim}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
% functions
\newcommand{\Ex}{\mathop{\bf E\/}}
\newcommand{\EV}{\mathbf{E}} % Bold E for expected value
\newcommand{\EVb}[1]{\EV\left\{#1\right\}} % EV with fitted  CURLY brackets
\newcommand{\EVs}[1]{\EV\left[#1\right]} % EV with fitted  SQUARE brackets
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\vspan}{\mathrm{span}}
\newcommand{\im}{\mathrm{im}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Flin}{\mathrm{F,lin}}
\newcommand{\mutG}{\mathrm{mut,G}}
\newcommand{\OLE}{\mathrm{OLE}}
\newcommand{\tnorm}[1]{\lVert#1\rVert_2}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\xvec}{\mathbf{x}}

% special variables
\newcommand{\taur}{\tau_\mathrm{ref}} % Absolute refractory period
\newcommand{\vth}{v_\mathrm{th}} % Threshold
\newcommand{\vres}{v_\mathrm{r}} % Reset % Note: do not use \vr - conflict with revtex
\newcommand{\rhoavg}{\rho^{\mathrm{avg}}}
\newcommand{\kaavg}{\kappa^{\mathrm{avg}}}
\newcommand{\rhoin}{\rho^{\mathrm{input}}}
\newcommand{\rhoout}{\rho^{\mathrm{output}}}
\newcommand{\rhosig}{\rho^{\text{sig}}}
% Motif frequencies
\newcommand{\dout}{d^{\mathrm{out}}}
\newcommand{\din}{d^{\mathrm{in}}}
\newcommand{\qdiv}{q_{\mathrm{div}}}
\newcommand{\qch}{q_{\mathrm{ch}}}
\newcommand{\qcon}{q_{\mathrm{con}}}
\newcommand{\Qdiv}{Q_{\mathrm{div}}}
\newcommand{\Qch}{Q_{\mathrm{ch}}}
\newcommand{\Qcon}{Q_{\mathrm{con}}}
\newcommand{\bfQdiv}{\mathbf{Q}_{\mathrm{div}}}
\newcommand{\bfQch}{\mathbf{Q}_{\mathrm{ch}}}
\newcommand{\bfQcon}{\mathbf{Q}_{\mathrm{con}}}
% terms
\newcommand{\IF}{IF }
\newcommand{\ER}{Erd\"{o}s-R\'{e}nyi}
\newcommand{\WK}{Wiener-Khinchin}
\newcommand{\OU}{Ornstein-Uhlenbeck}




